Detecting Adversarial Examples in Learning-Enabled Cyber-Physical Systems using Variational Autoencoder for Regression

Learning-enabled components (LECs) are widely used in cyber-physical systems (CPS) since they can handle the uncertainty and variability of the environment and increase the level of autonomy. However, it has been shown that LECs such as deep neural networks (DNN) are not robust and adversarial examples can cause the model to make a false prediction. The paper considers the problem of efficiently detecting adversarial examples in LECs used for regression in CPS. The proposed approach is based on inductive conformal prediction and uses a regression model based on variational autoencoder. The architecture allows to take into consideration both the input and the neural network prediction for detecting adversarial, and more generally, out-of-distribution examples. We demonstrate the method using an advanced emergency braking system implemented in an open source simulator for self-driving cars where a DNN is used to estimate the distance to an obstacle. The simulation results show that the method can effectively detect adversarial examples with a short detection delay.

==> method_mod.tex <==
\section{Variational Autoencoder for Regression and Adversarial Examples Detection}
\label{sec:method}
In this section, we propose a detection method based on inductive conformal prediction~\cite{laxhammar2015inductive} for a Variational Autoencoder (VAE) based regression model~\cite{zhao2019variational} that extends the work in~\cite{CaiICCPS20}.
The inductive conformal prediction is  used to generate a nonconformity score of the perception input based on the reconstruction error of the VAE  comparing to the reconstruction error of the training examples to measure the trustworthy of the input.
In the following, we introduce the detection system in details.

\subsection{Variational Autoencoder for Regression}
A VAE is a generative model whose encodings' distribution is regularised during the training in order to ensure that its latent space has good properties allowing the generation of new data\cite{DBLP:journals/corr/KingmaW13}. 
The objective is to model the relationship between the observation $x$ and the low-dimensional latent variable $z$. The architecture presented in~\cite{zhao2019variational} integrates a regression model into the generative model 
to disentangle the regression target variable from the latent space. The architecture of the VAE-based regression model is shown in Fig.~\ref{fig:model}. 

\begin{figure}[!ht]
	\centering
	\input{./figures/model.tex}
	\caption{VAE-based regression model\cite{zhao2019variational}.}
	\label{fig:model}
\end{figure}  

Similar to a traditional VAE, the encoder attempts to represent the input on the latent space using a Gaussian distribution $p(z)$. Instead of using a single Gaussian prior, the VAE-based regression model conditions the prior on the regression target variable $c$ such that the new prior $p(z|c)$, called \textit{latent generator}, can be used to sample a specific latent representation for a given target variable $c$. 
%On the other branch of the architecture, a regression network $q(c|x)$ with  additional output uncertainty of the prediction is used to inference the target variable. % XK: Are you sure about this sentence?
On the other branch of the architecture, a regression network $q(c|x)$ is used to infer the target variable and its uncertainty.
The total loss for the VAE based regression is defined as 
\begin{equation*} \label{eq:vaeLoss}
\begin{split}
\mathcal{L}(\theta, \phi_c, \phi_z; x) = &- D_{\text{KL}}(q_{\phi_c}(c|x) || p(c))\\
&+   \mathbb{E}_{z\sim q_{\phi_z}(z|x)}[\log p_\theta(x|z)]\\
&- \mathbb{E}_{c\sim q_{\phi_c}(c|x)}[ D_{\text{KL}}(q_{\phi_z}(z|x)||p(z|c))],
\end{split}
\end{equation*}
where $\theta$, $\phi_{z}$ and $\phi_{c}$ are the neural network parameters. The first term regularizes the prediction of $c$ with a ground-truth prior $p(c)$. The second term is the model fit trying to reconstruct the input from the latent representations. The third term is the KL divergence between the approximate posterior and the regression-specific prior $p(z|c)$. 
Both the VAE and the regression model can be trained as a single network and the target variable is disentangled from the latent space.

\subsection{Adversarial Examples for Regression Model}
A common approach to generate adversarial examples is the fast gradient sign method (FGSM)~\cite{goodfellow2014explaining}, which computes an adversarial input by adding a small perturbation making the prediction move towards the reversed direction of the gradient descent.
Usually, FGSM is used for classification problems. In this work, we apply this method to generate adversarial examples for regression neural network that can cause large output error.


For a given input $x$ and a target output $y^{\text{target}}$, the neural network output is the regression estimation $c = f(x)$. The objective is to change $x$ to $\tilde{x}$ such that the error between $y^{\text{target}}$ and $f(\tilde{x})$ is minimized, which can be formulated by  $J(\tilde{x}, y^{\text{target}}) = |f(\tilde{x}) - y^{\text{target}} |^2$.


\subsection{Adversarial Detection}
In this subsection, we introduce inductive conformal prediction (ICP)\cite{balasubramanian2014conformal} method for anomaly detection. First, we discuss a general framework for conformal prediction. Next, we show how we define nonconformity score based on VAE's output and use it for anomaly detection.
\subsubsection{Conformal prediction}
\label{sec:cp}
The core idea of the method is the \textit{nonconformity measure} defined by a function $A$ that assigns a value as \textit{nonconformity score} indicating how different a test example is from the training data set. A large nonconformity score corresponds to a strange example with respect to the training data set. The original training set $\{ (x_1,y_1), \ldots, (x_l, y_l)\}$ is split into a proper training set $\{ (x_1,y_1), \ldots, (x_m, y_m)\}$ and a calibration set $\{ (x_{m+1},y_{m+1}), \ldots, (x_l, y_l)\}$. For each calibration example, the nonconformity scores $\alpha_{m+1}, \ldots, \alpha_{l}$ are precomputed relative to the proper training set. 
For a test example $(x^\prime_{k}, y^\prime_{k})$, the nonconformity score $\alpha^\prime_{k}$ is computed using the same way relative to the proper training set and the $p$-value is defined as the fraction of calibration examples that have nonconformity scores greater than or equal to the $\alpha^\prime_{k}$
\begin{equation}
p_k = \frac{|\{i=m+1, \ldots, l\} \, | \, \alpha_i \geq \alpha^\prime_k|}{l-m}.
\label{eq:p-value}
\end{equation}
If the $p$-value is smaller than a predefined threshold $\epsilon \in (0,1)$, the test example can be classified as a conformal anomaly. Using a single $p$-value for detecting the anomaly will make the detector oversensitive.
The robustness of the detector can be considerably improved if multiple $p$-values are used.
In \cite{vovk2005algorithmic}, it  is shown that if the test examples are independent and identically distributed (IID) , the $p$-values are independent and uniformly distributed in $[0,1]$.
Further, a martingale test is used to test the hypothesis that the  $p$-values are independent and uniformly distributed,  and the martingale value is used as an indicator for the unusual test example~\cite{vovk2005algorithmic}. 
in~\cite{Fedorova:2012:PMT:3042573.3042693}, the \textit{simple mixture martingale} is used which is defined as 
\begin{equation}
M = \int_{0}^{1}\prod_{i=1}^{N}\epsilon p_i^{\epsilon-1}d\epsilon.
\label{eq:martingale}
\end{equation}
$ M $ will grow only if there are many small $p$-values in the sequence. More details about the martingales can be found in~\cite{Fedorova:2012:PMT:3042573.3042693}. 

Given the VAE model, we can rely on it  to generate multiple examples sampling from the learned latent space probability distribution. The samples which are similar to the input are IID and can be used to generate $p$-values that are independent and uniformly distributed in $[0,1]$. Then, the martingale can be used to test this hypothesis and detect if the test example comes from the training data set distribution. 
Next, we explain how we compute the nonconformity score.


\subsubsection{Nonconformity measure and adversarial detection algorithm}
In work~\cite{CaiICCPS20}, the reconstruction error (squared error between the input $x$ and the generated output $\hat{x}$) of VAE model is used as the nonconformity measure
\begin{equation*}
\alpha = A_{\text{VAE}}(x, \hat{x}) = ||x-\hat{x}||^2.
\end{equation*}
In this paper, we use the same nonconformity measure based on the output of the VAE-based regression model which integrates the regression model and the VAE (Fig.~\ref{fig:model}). 

During the offline phase, 
the training set $\{ (x_1, y_1),  \ldots, (x_l, y_l)\}$ is split into a proper training set $\{ (x_1, y_1),  \ldots, (x_m, y_m)\}$ and a calibration set $\{ (x_{m+1}, y_{m+1}),  \ldots, (x_l, y_l)\}$. 
%In~\cite{CaiICCPS20}, two independent models are trained for regression and nonconformity measure separately. In this work, 
The VAE-based regression model is trained by utilizing the proper training data set.
%which combines the regression and the nonconformity measure in a single model. 
For each example in the calibration data set, the nonconformity score is precomputed using the 
nonconformity measure $A_{\text{VAE}}$.
 
At runtime, a sequence of test inputs $(x_1^\prime, \ldots, x_t^\prime, \ldots)$ is processed one-by-one. 
%and they are time-correlated, and therefore not independent. In order to satisfy the exchangeability assumption,  
Consider the input $x^\prime_t$. The method samples from the posterior distribution of the latent space to generate $N$ new examples $\hat{x}_{t,1}^\prime, \ldots, \hat{x}_{t,N}^\prime$, and
the nonconformity score $\alpha^\prime_{t,k}$ and the corresponding $p$-value for each generated example $\hat{x}_{t,k}^\prime$ are computed using $A_{\text{VAE}}$ and Eq.~(\ref{eq:p-value}).  
Since the generated examples are IID, the $p$-values $(p_{t,1}, \ldots, p_{t,N})$ are independent and uniformly distributed in $[0,1]$. Therefore, the martingale in Eq.~(\ref{eq:martingale}) can be used for detection.
The martingale denoted by $M_t$ has a large value if there are many small $p$-values in the sequence $(p_{t,1}, \ldots, p_{t,N})$ which indicates an out-of-distribution input. 

In order to robustly detect when the martingale becomes consistently large, \cite{CaiICCPS20} uses a stateful CUSUM (Cumulative Sum) detector to generate alarms for out-of-distribution inputs by keeping track of the historical information of the martingale values. 
The detector is defined as $S_1=0$ and $S_{t} = \max(0, S_{t-1} + M_{t-1} - \delta)$,  
where $\delta$ prevents $S_t$ from increasing consistently when the inputs are 
in the same distribution as the training data. An alarm is raised whenever $S_t$ is 
greater than a threshold $S_t > \tau $ which can be optimized using empirical
data~\cite{basseville1993detection}. Typically, after an alarm the test is 
reset with $ S_{t+1} = 0$.
%
Algorithm~\ref{alg:vae} describes the steps of the method. 

\begin{algorithm}[!ht]
	\caption{Adversarial examples detection using the VAE-based regression model}
	\label{alg:vae}
	\begin{algorithmic}[1]
		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
		\renewcommand{\algorithmicensure}{\textbf{Output:}}
		\REQUIRE Input training set $\{ (x_1, y_1),  \ldots, (x_l, y_l)\}$, test examples $(x^\prime_1, \ldots, x^\prime_t, \ldots)$, number of calibration examples $l-m$, 
		number of examples to be sampled $N$, 
		stateful detector threshold $\tau$ and parameter $\delta$
		\ENSURE  Output boolean variable $Anom_{t}$, regression result $c_t$
		
		\renewcommand{\algorithmicrequire}{\textbf{Offline:}}
		\renewcommand{\algorithmicensure}{\textbf{Online:}}
		
		\REQUIRE 
		\STATE Split the training set $\{ (x_1, y_1),  \ldots, (x_l, y_l)\}$ into the proper training set $\{ (x_1, y_1),  \ldots, (x_m, y_m)\}$ and calibration set $\{ (x_{m+1}, y_{m+1}),  \ldots, (x_l, y_l)\}$
		\STATE Train a VAE-based regression model $f(\cdot)$ using the proper training set and get the corresponding nonconformity measure $A_{\text{VAE}}(\cdot)$
		\FOR {$j = m+1$ to $l$}
		\STATE Sample $\hat{x}_j$ using the trained VAE
		\STATE $ \alpha_j = A_{\text{VAE}}(x_j, \hat{x}_j) $
		\ENDFOR
		
		\ENSURE
		\FOR {$t = 1, 2, \ldots$}
		\FOR {$k = 1$ to $N$}
		\STATE Sample $ \hat{x}^\prime_{t,k} $ using the trained VAE
		\STATE $\alpha^\prime_{t,k} = A_{\text{VAE}}(x^\prime_t,\hat{x}^\prime_{t,k})$
		\STATE $p_{t,k} = \frac{|\{i=m+1,\ldots,l\} \,|\, \alpha_i \geq \alpha^\prime_{t,k}|}{l - m}$ 
		\ENDFOR
		\STATE $M_t =  \int_0^1 \prod_{k=1}^N \epsilon p_{t,k}^{\epsilon - 1} d\epsilon$
		\IF {$t=1$} 
		\STATE $S_t = 0$
		\ELSE
		\STATE $S_t = \max(0, S_{t-1} + M_{t-1} -\delta)$
		\ENDIF
		\STATE $Anom_{t} \leftarrow S_t > \tau $
		\STATE $c_t = f(x^\prime_t)$ 
		\ENDFOR
	\end{algorithmic} 
\end{algorithm}
